Low Frequency Adversarial Perturbation

Adversarial images aim to change a target model's decision by minimally perturbing a target image. In the black-box setting, the absence of gradient information often renders this search problem costly in terms of query complexity. In this paper we propose to restrict the search for adversarial images to a low frequency domain. This approach is readily compatible with many existing black-box attack frameworks and consistently reduces their query cost by 2 to 4 times. Further, we can circumvent image transformation defenses even when both the model and the defense strategy are unknown. Finally, we demonstrate the efficacy of this technique by fooling the Google Cloud Vision platform with an unprecedented low number of model queries.

==> motivation.tex <==
%!TEX root=./main.tex

%Figure \ref{fig:dct_spectrum} shows the effect on cosine wave coefficients after applying JPEG compression to natural images. For an image $\bx$, let $\bx'$ be the corresponding image compressed using JPEG. Let $\bv = \dct(\bx)$ and $\bv' = \dct(\bx')$ be the frequency space representation of the two images, where $\dct$ is applied independently across the color channels. The relative difference $|\bv - \bv'|/|\bv|$ is shown in log scale. Negative values indicate little to no relative change in the coefficient, while positive values indicate large relative change. Note that most of the large changes occur in high frequency coefficients.

%We discover that a particular class of defense strategy is surprisingly effective against the boundary attack. Image transformation defenses \citep{dziugaite2016study, xu2017feature, guo2017countering} aim to remove or reduce adversarial perturbations by image compression techniques such as JPEG and total variation minimization. These transformations affect the decision boundary of the model by quantizing the image space into regions where all images in the region are roughly equal after transformation. This has an adverse effect on the boundary attack since it relies on a smooth decision boundary \citep{brendel2017decision}.
%Since each step of the boundary attack involves adding small Gaussian noise to the current iterate, most iterates would result in no change to the image after transformation. The change will only be reflected after stacking a large number of iterations, which forces the model to take steps blindly without meaningful feedback on success.

%\begin{figure}
%\centering
%\begin{minipage}{.45\textwidth}
%  \centering
%  \includegraphics[width=\textwidth]{fig/ba_succ.pdf}
%	\vspace{-1em}
%	\caption{Average success rate of the boundary attack against various defenses. The attack fails to approach the target image due to effects of image transformations.}
%	\label{fig:ba_succ}
%\end{minipage}%
%\qquad
%\begin{minipage}{.45\textwidth}
%  \centering
  %\includegraphics[width=\textwidth]{fig/ba_failure_modified.pdf}
%  \includegraphics[width=\textwidth]{fig/ba_failure.pdf}
%	\caption{Example of a failed run of the boundary attack against JPEG defense. The leftmost image is a clean image of a correctly classified redshank bird. The middle and rightmost images are adversarial images constructed by the boundary attack against no defense and JPEG compression, respectively. The JPEG defense forces the attack to add clearly visible noise. (Zoom in for details.)}
%	\label{fig:ba_failure}
%\end{minipage}
%\end{figure}

%Figure \ref{fig:ba_succ} shows the average success rate across iterations of the boundary attack applied to a ResNet-50 network \citep{he2016residual}. An attack is considered successful if the perturbed image has a mean squared error (MSE) of $\leq 0.001$ from the clean image. We evaluate the following deterministic image transformation defenses:
%\begin{itemize}[noitemsep]
%\item JPEG compression \citep{dziugaite2016study} at quality level 75;
%\item Reducing bit depth (i.e., quantization) \citep{xu2017feature} to 3 bits; and
%\item Total variation minimization \citep{guo2017countering} with weight 0.1.
%\end{itemize}

%Against both the JPEG and bit reduction defenses, the boundary attack fails to make progress, while against the TV minimization defense, success rate increase is dramatically slower. Figure \ref{fig:ba_failure} shows a sample image (leftmost), and adversarial images produced by the boundary attack against no defense (middle) and the JPEG defense (rightmost). The perturbation added is clearly more visible when JPEG defense is applied.

